Watermarking Text Generated by Black-Box Language Models

LLMs now exhibit human-like skills in various fields, leading to worries about misuse. Thus, detecting generated text is crucial. However, passive detection methods are stuck in domain specificity and limited adversarial robustness. To achieve reliable detection, a watermark-based method was proposed for white-box LLMs, allowing them to embed watermarks during text generation. The method involves randomly dividing the model vocabulary to obtain a special list and adjusting the probability distribution to promote the selection of words in the list. A detection algorithm aware of the list can identify the watermarked text. However, this method is not applicable in many real-world scenarios where only black-box language models are available. For instance, third-parties that develop API-based vertical applications cannot watermark text themselves because API providers only supply generated text and withhold probability distributions to shield their commercial interests. To allow third-parties to autonomously inject watermarks into generated text, we develop a watermarking framework for black-box language model usage scenarios. Specifically, we first define a binary encoding function to compute a random binary encoding corresponding to a word. The encodings computed for non-watermarked text conform to a Bernoulli distribution, wherein the probability of a word representing bit-1 being approximately 0.5. To inject a watermark, we alter the distribution by selectively replacing words representing bit-0 with context-based synonyms that represent bit-1. A statistical test is then used to identify the watermark. Experiments demonstrate the effectiveness of our method on both Chinese and English datasets. Furthermore, results under re-translation, polishing, word deletion, and synonym substitution attacks reveal that it is arduous to remove the watermark without compromising the original semantics.

==> abstract.tex <==


% Original
% Large language models have reached human-level performance on various professional and academic benchmarks. This has sparked concerns of malicious applications, such as spreading misinformation and cheating in school assignments. Consequently, detecting and auditing the generated text has become crucial. Existing post-hoc detection approaches, relying on training classifiers to capture detectable features in generated text, are hindered by domain specificity and limited adversarial robustness. 
% % As language models continue to advance, the challenge of differentiating between human-authored and machine-generated text is expected to intensify. 
% In light of this, a watermark-based detection method was proposed by randomly dividing the model vocabulary to obtain a set of tokens and encouraging the model to incorporate them at each token generation step. However, it necessitates control over the probability distribution over the vocabulary, which is often unattainable, as service providers may only offer APIs without the probability distribution to protect commercial interests. 

% Considering that third parties developing downstream services based on APIs (e.g., AutoGPT) also need to detect, audit, or protect the copyright of their generated texts, we propose a watermarking framework for the black-box scenario by embedding an identification watermark in the already generated text. Specifically, we generate context-based synonyms for a portion of words in the original text and select the synonym to replace the corresponding original word with our random synonym sampling algorithm. We then employ a statistical test to detect the watermark. Experimental results demonstrate that our algorithm has good performance on Chinese and English datasets, with robustness against attacks such as synonym substitution, word deletion, re-translation, and GPT-3.5-based polishing.

% version 4.21
Large language models now show human-like skills in different fields, leading to worries about misuse like spreading misinformation and enabling academic dishonesty. Thus, detecting generated text is crucial. However, passive detection methods that train classifiers to identify generated text, are stuck in domain specificity and limited adversarial robustness. 
% face challenges in domain specificity and adversarial robustness. 
To achieve reliable diagnosis, a watermark-based method was proposed for white-box language models, allowing them to embed watermarks during text generation.
% by selecting more words in a special list than would be expected in human-written text.
The method involves randomly dividing the model's vocabulary to obtain a special list and adjusting the output probability distribution to
% It randomly divide the model vocabulary to obtain the special list and adjusting the output probability distribution to 
promote the use of words in the list at each generation step. A detection tool aware of the special list can distinguish between watermarked and non-watermarked text.
% However, this method is not accessible to third-party developers creating downstream services based on model APIs, as API providers often withhold the probability distribution information to safeguard their commercial interests.
However, this method is not applicable in many real-world scenarios where only black-box language models are available.
For instance, third-parties that develop API-based vertical applications cannot watermark text themselves because API providers only supply generated text and withhold probability distributions to protect their commercial interests.

% Given the need for third parties to detect or authenticate text generated from them, we propose a watermarking framework that injects authentication watermarks  into the already generated text from black-box language models. 
% To enable users of black-box language models to autonomously embed watermarks in text, 
To enable third-parties to autonomously inject watermarks into generated text, we propose a watermarking framework for black-box language model usage scenarios. 
% Specifically, we generate context-based synonyms for selected words in the original text and replace them with the synonyms chosen by our watermark-driven synonym sampling algorithm. A statistical test is then used to detect the watermark. 
Specifically, we first define a binary encoding function to compute a random binary encoding corresponding to a word. The encodings computed for non-watermarked text conform to a Bernoulli distribution, wherein the probability of a word representing bit-1 being approximately 0.5.
To inject a watermark, we alter the distribution by selectively replacing words representing bit-0 with context-based synonyms that represent bit-1. A statistical test is then used to identify the watermark. 
Experiments demonstrate the effectiveness of our method on both Chinese and English datasets. 
Furthermore, results under sentence re-translation, sentence polishing, word deletion, and synonym substitution attacks reveal that it is arduous for attackers to remove the watermark without compromising the original semantics.
% robustness tests under sentence-level and word-level attacks indicate that it is tough for attackers to erase the watermark without compromising the original semantics.


% However, it necessitates control over the probability distribution over the full vocabulary. which may be inaccessible as service providers often only provide APIs without the probability distribution to safeguard their commercial interests.

% Large language models now show human-like skills in different fields, leading to worries about misuse like spreading misinformation and enabling academic dishonesty. Thus, detecting generated text is crucial. However, passive detection methods that train classifiers to identify generated text, are stuck in domain specificity and limited adversarial robustness. To achieve reliable diagnosis, a watermark-based method was proposed for white-box language models, allowing them to embed watermarks during text generation. The method involves randomly dividing the model's vocabulary to obtain a special list and adjusting the output probability distribution to promote the use of words in the list at each generation step. A detection tool aware of the special list can distinguish between watermarked and non-watermarked text. However, this method is not applicable in many real-world scenarios where only black-box language models are available. For instance, third-parties that develop API-based vertical applications cannot watermark text themselves because API providers only supply generated text and withhold probability distributions to protect their commercial interests. To enable third-parties to autonomously inject watermarks into generated text, we propose a watermarking framework for black-box language model usage scenarios. Specifically, we first define a binary encoding function to compute a random binary encoding corresponding to a word. The encodings computed for non-watermarked text conform to a Bernoulli distribution, wherein the probability of a word representing bit-1 being approximately 0.5. To inject a watermark, we alter the distribution by selectively replacing words representing bit-0 with context-based synonyms that represent bit-1. A statistical test is then used to identify the watermark. Experiments demonstrate the effectiveness of our method on both Chinese and English datasets. Furthermore, results under sentence re-translation, sentence polishing, word deletion, and synonym substitution attacks reveal that it is arduous for attackers to remove the watermark without compromising the original semantics.


% Watermarked 
% Large language models (e.g., ChatGPT) have exhibited human-level performance on various professional and academic benchmarks. However, this has severely sparked concerns about the misuse of the generated texts, such as spreading misinformation and cheating in academic writing and school assignments. Consequently, detecting and auditing the generated text has become crucial. Existing passive detection approaches, relying on training classifiers, are hindered by domain specificity and limited adversarial robustness. In light of this, a watermark-based active detection method was proposed by split the model vocabulary to obtain a set of tokens and encouraging the model to incorporate them during the sampling process. However, it necessitates authority over the model' s output, which is sometimes unattainable, as service providers may only sell APIs without full distributions to shield business interests. 

% Considering that third parties developing downstream services based on APIs additionally need to identify, audit or protect the copyright of their generated texts, we propose a watermarking framework for the black-box scenario by embedding an identification watermark in the already generated text. Specifically, we create context-based synonyms for a portion of words in the original text and select the synonym to replace corresponding original term with our random synonym sampling algorithm. We then utilize a statistical test to identify the watermark. Experimental results demonstrate that our algorithm has good performance on Chinese and English datasets, with robustness against attacks such as synonym substitution, word deletion, re-translation, and GPT-3.5-based polishing.

==> figures/overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/overview_fig.pdf}
    \caption{An illustration of \tool, which enables 
	     homomorphically encrypted neural network inference with guarantees. The
	     symbol~\protect\lock denotes encryption of the value in an \fhe scheme
	     by the client.}
    \label{fig:overview}
\end{figure*}


==> src/app_eval.tex <==
\section{Full Experimental Details} \label{app:eval} Here we list all details of
our evaluation that were omitted from \cref{sec:eval}.

In all \toolR experiments we use the following parameters for \textsc{ArgmaxHE}:
\mbox{$d_q^{(1)}=6, d_p^{(1)}=1, d_q^{(2)}=2, d_p^{(2)}=2$}, use the largest
batch size supported, $B=32$, and set $\alpha=0.001$. For MNIST, we use the
randomized smoothing parameters $\sigma=0.5$, $n=128$, $n_0=32$,
$\tau=0.76=0.75+\zeta$ where $\zeta=0.01$. For CIFAR, we use $\sigma=0.25$,
$n=64$, $n_0=8$, and as before, $\tau=0.76$.
 
For the \toolF (Adult dataset) experiment presented in
\cref{ssec:eval:smoothing}, we use \mbox{$d_q^{(1)}=6, d_p^{(1)}=0, d_q^{(2)}=0,
d_p^{(2)}=2$}. Setting \mbox{$d_p^{(1)}=d_q^{(2)}=0$} is enabled by the special
case of binary classification ($c=2$) which is common in fairness problems. We
use $\alpha = 0.001$, and set the maximum $B=1024$ and \mbox{$n=n_0=1024$}
enabled by the setting (1 batch each for the preliminary and the main count).
The similarity constraint $\theta$ is manually set by inspecting the attributes,
\eg we set $\theta_{i}=2$ for the age attribute, and $\theta_{i}=1$ for the
education level. The $\Sigma$ covariance matrix obtained from $\theta$ is used
to add Gaussian noise to batches of examples during training. 
\balance
Note that we can obtain an equivalent formulation of our problem (see
\cref{eq:robustness2}) by multiplying $\Sigma$ by a constant factor $\kappa$ and
dividing $R = \sqrt{1/L}$ by the same factor, which introduces a tradeoff. While
smaller $R$ leads to smaller $\tau$ and is thus easier to certify, it introduces
$\Sigma$ with larger total variation. This in turn increases the noise that is
used in both training and certification, making it harder to obtain correct
predictions for samples used in the process of randomized smoothing. In our
implementation we rescale $\Sigma$ to total variation of $\kappa d$, where we
try several values of $\kappa$ and choose $\kappa = 0.5$, based on the
accuracy-certifiability tradeoff. This leads to $\tau = \Phi(\sqrt{1/L}) + \zeta
= 0.719$ (as $\zeta=0.01$ as before).

==> src/app_harm.tex <==
\subsection{Harmless Violations} \label{app:harm} Here we provide more details
on the distinction between harmless and harmful violations introduced in
\cref{ssec:eval:warmup}.

Recall from \cref{sec:error} that \textsc{SgnHE} requires each logit vector $z
\in \mathbb{R}^c$ to satisfy
\begin{itemize} 
    \item $\forall i\colon\ z_i \in [Z_\textit{min}, Z_\textit{max}]\ $ (\emph{range
    condition}), and
    \item $\forall i \neq j\colon\ |z_i-z_j| \geq D\ $ (\emph{difference
    condition}),
\end{itemize}
for some chosen constants $Z_\textit{min}, Z_\textit{max}, D$.   
As long as it holds that \mbox{$\max(z) - \min(z) \leq Z_\textit{max} - Z_\textit{min}$} and
$z_1 - z_2 \geq D$, where $z_1$ and $z_2$ are the two largest logits, the result
will not be inconsistent. We call violations that satisfy these conditions
\emph{harmless}. We next illustrate this behavior on the example of difference
violations, as their analysis is more involved.

Intuitively, harmless difference violations exist as invalidating the input
requirement of the first invocation of \textsc{SgnHE} (\cref{lin:argmax:sign-1}
in \cref{alg:argmax}) can in some cases still lead to the input requirement for
the second invocation being satisfied (\cref{lin:argmax:sign-2}), implying that
the final result of \textsc{ArgmaxHE} will not be affected.


More formally, as derived in \appref{app:params}, the difference condition
implies a certain input requirement parameter $\phi^{(1)}$ for the first
\textsc{SgnHE} invocation (\cref{lin:argmax:sign-1} in \cref{alg:argmax}). From
there, we carefully derived $d_q^{(1)}$ and $\psi^{(1)}$ such that
\textsc{SgnHE} is provably $(\phi,\psi)$-close, as defined in
\cref{sec:argmaxhe}.
This allows us, assuming no violations, to reason about the values of
$\mathit{scores}$ and transform its first $c$ slots to \mbox{$[-1, \ldots,
-1/(2c-2), 1/(2c-2)]$} (\cref{lin:argmax:scores}), before invoking the second
\textsc{SgnHE} (\cref{lin:argmax:sign-2}).

If there is a harmless violation, for example $z_{c} - z_{c-1} > -D$ (where
$z_{c}$ and $z_{c-1}$ are the smallest and the second smallest logit in~$z$),
the input requirement $\phi^{(1)}$ is violated, making the $(\phi,\psi)$-close
guarantee invalid. However, while the output of the first \textsc{SgnHE} for the
entry in $\mathit{diff}$ corresponding to $z_{c} - z_{c-1}$ is not anymore
guaranteed to be close to $-1$ it will still be in the range $[-1, 0]$. Thus,
the element of $\mathit{scores}$ corresponding to $z_{c}$ will not be
approximately $-1$ (after \cref{lin:argmax:scores}) as before, but will be
provably below $-1/(2c-2)$. This implies that the behavior of the second
\textsc{SgnHE} will remain unchanged and will map that element to $-1$ with
usual approximation error. An analogous argument can be made for other
difference violations, showing that only $z_1-z_2 < D$ is a harmful difference
violation that can affect the result of \textsc{ArgmaxHE}.


==> src/app_params.tex <==
\subsection{Parameter Choice Procedure} \label{app:params} In \cref{sec:error}
we derived an upper bound on the error probability of our system. In this
section, we describe a previously referenced procedure that jointly chooses the
condition parameters \mbox{$(Z_\textit{min}, Z_\textit{max}, D)$}, the \textsc{ArgmaxHE}
parameters \mbox{$(d_{q}^{(1)}$, $d_{p}^{(1)}$, $d_{q}^{(2)}$, $d_{p}^{(2)})$}
and the precision settings $(\phi^{(1)}, \psi^{(1)}, \phi^{(2)}, \psi^{(2)})$
for two \textsc{SgnHE} invocations, such that the obtained guarantees hold if
the range and difference conditions hold (up to the algorithmic error, the
probability of which is by construction at most $\alpha$).
   
\para{Choosing $Z_\textit{min}$ and $Z_\textit{max}$} To choose the range $[Z_\textit{min}, Z_\textit{max}]$
we propagate all examples $x$ from the training set through the network $f$ to
obtain the logit vectors $z = f(x)$, and keep $50$ examples with largest
$\max(z)$, $50$ with smallest $\min(z)$ and $100$ with the largest $\max(z) -
\min(z)$. On these $200$ examples we run two PGD adversarial attacks
\cite{MadryMSTV18} with $\ell_2$ radius $R=2$, and $100$ steps of size $0.01$, to
obtain adversarial examples $\hat{x}$ from $x$ that maximize (resp. minimize)
the extreme $z_i$. Next, we $n$ times sample and add Gaussian noise
$\varepsilon_i \sim \mathcal{N}(0, \sigma)$ to each $\hat{x}$ and note the
largest and the smallest observed value of $z_i \in z = f(\hat{x} +
\varepsilon_i)$. Finally, we add a small margin to the obtained result to obtain
the final values for $[Z_\textit{min}, Z_\textit{max}]$.

\para{Ensuring the \textsc{SgnHE} Input Requirement} Before proceeding, we comment on
the basic input requirement of \textsc{SgnHE}, namely that its inputs are in $[-1,
1]$. To ensure this requirement for the first invocation
(\cref{lin:argmax:sign-1} in \cref{alg:argmax}), we normalize all logits:
\begin{equation*}
    \hat{z}_i = (z_i - Z_\textit{min}) / (Z_\textit{max} - Z_\textit{min}).
\end{equation*}
In practice, this is done by modifying the weight of the last layer of the
neural network. Note that under the range condition $z_i \in [Z_\textit{min}, Z_\textit{max}]$
(\cref{sec:error}), it is ensured that the normalized logits are in $[0, 1]$,
meaning that for all $i \neq j$ it is $\hat{z}_i -\hat{z}_j \in [-1, 1]$,
satisfying the requirement of the first invocation of \textsc{SgnHE}, invoked
on logit differences. The input requirement of the second invocation
(\cref{lin:argmax:sign-2}) holds by construction, as the input $\mathit{scores}$
is guaranteed to contain values in $[-1, 1/(2c-2)]$ (and trivially $c \geq 2$).

\para{Setting $d_q^{(1)}$ and $D$} We proceed to choose the parameters of
\textsc{ArgmaxHE} used in \textsc{SgnHE} invocations. To this end, we
extensively use the Lemma 3 from~\cite{CheonKK20} to find the minimal
$d_q(\phi)$ for a given input guarantee $\phi$, where smaller $d_q$ requires a
larger $\phi$. Similarly, we use Lemma 4 from the same paper to find the minimal
$d_p(\psi)$ for the required output precision $\psi$, where for larger $\psi$ we
need a larger $d_p$.

As the first \textsc{SgnHE} is applied to logit differences we have that
$\phi^{(1)} = D / (Z_\textit{max} - Z_\textit{min})$, where $D$ is smallest absolute
difference of two logits before normalization, per the difference condition
(\cref{sec:error}). This introduces a tradeoff when choosing $d_q^{(1)}$.
Namely, reducing $d_q^{(1)}$ (to reduce multiplicative depth and reduce latency)
requires ensuring a larger $D$ and makes it more probable that the difference
condition is violated. We choose $d_q^{(1)}=6$ which implies a particular value
of $D$ in each of our applications. 

\para{Setting $d_p^{(1)}$ and $d_q^{(2)}$} The parameters $d_p^{(1)}$ and
$d_q^{(2)}$ are directly dependent on each other. For fixed $\psi^{(1)}$, after
normalization (\cref{lin:argmax:scores} in \cref{alg:argmax}) the smallest
absolute value of an element of $\mathit{scores}$, the input to second
\textsc{SgnHE}, can be calculated as
\begin{equation*}
    \phi^{(2)} = (1 - (c-1)2^{-\psi^{(1)}}) / (2c-2).
\end{equation*}
Increasing $\psi^{(1)}$ (by increasing $d_p^{(1)}$) leads to larger
$\phi^{(2)}$, allowing smaller $d_q^{(2)}$, inducing a tradeoff. For the trivial
condition $\phi^{(2)}>0$ we need $\psi^{(1)} > \log(c-1)$. Similarly, we see
that $\phi^{(2)} \leq 1/(2c-2)$. 

We could do a linear search to find the minimal $d_p^{(1)}+d_q^{(2)}$. However,
in all cases we consider the two stated conditions imply $d_p^{(1)} \geq 1$ and
$d_q^{(2)} \geq 2$, and we can see that $d_p^{(1)}=1, d_q^{(2)}=2$ are in fact
simultaneously achievable, guaranteeing \mbox{$\psi^{(1)} \approx 6$} and in
turn \mbox{$\phi^{(2)} \approx 0.05$}. However, $d_q^{(2)}=2$ supports
$\phi^{(2)} \geq 0.0423$, providing additional room for error.

\para{Setting $d_p^{(2)}$} Randomized smoothing, used to derive robustness and
fairness guarantees in \cref{sec:smoothing}, concludes by summing up $n$ outputs
of the second \textsc{SgnHE} (divided by two) and expects the client to
correctly round up the sums to the nearest integer. Therefore, we require $n \cdot 2^{-\psi^{(2)}} / 2 < 0.5$, \ie $\psi^{(2)} > \log(n)$. We can check that for
$d_p^{(2)}=1$ we can afford $n \leq 64$, but $d_p^{(2)}=2$ supports $n \geq
10^6$, which is more than sufficient for practical cases. $\psi^{(2)}$ that is
ensured by this choice is $26$, implying again that for realistic choices of $n$
there is a large margin preventing rounding errors.


==> src/app_reducing.tex <==
\subsection{Using Less Polynomial Evaluations} \label{app:reducing}

\input{tables/app_reducing}
The parameter values determining the number of polynomial evaluations within the
\textsc{SgnHE} approximation that we describe in \appref{app:params} and use in
all our main experiments in \cref{sec:eval} are carefully chosen to ensure no
errors caused by the approximation under stated conditions, and enable rigorous
upper bounding of the error probability~(\cref{sec:error}). In this section, we
explore how reducing the number of evaluations below the theoretically sound
values affects the results of the algorithm in practice.

\para{Setup} To investigate this, we repeat the \toolR experiments with the main
MNIST model from \cref{ssec:eval:smoothing} using MockSEAL with various values
of $d_{q}^{(1)}$, $d_{p}^{(1)}$, $d_{q}^{(2)}$, $d_{p}^{(2)}$. We show the
\emph{CountsOK} and \emph{ResultOK} columns, the percentage of examples where
the FHE evaluation obtained counts consistent with the non-private evaluation,
and where the final result (``abstain'' or ``guaranteed class $k$'') was
consistent. Our baseline are the theoretically sound choices of $d_q^{(1)}=6,
d_p^{(1)}=1, d_q^{(2)}=2, d_p^{(2)}=2$ for which the result for all $100\%$ of
examples is consistent.

\para{Results} The results are presented in \cref{table:reducing}. We can notice
that reducing $d_p^{(1)}$ or $d_q^{(2)}$ is impossible without greatly
sacrificing the quality of the results. On the other hand, we see that it is
possible to reduce $d_p^{(2)}$ to $1$ (but not to $0$), as well as significantly
reduce $d_q^{(1)}$ without a large effect on the result. While the percentage of
consistent counts slowly degrades as we decrease the parameters, the percentage
of consistent final results is more slowly affected, again demonstrating the
ability of the aggregation of predictions to absorb inaccuracies. 

While it is most often crucial to have formal guarantees given by the error
probability bounds, we can conclude that when this is not the case, using
significantly smaller parameters (thus significantly reducing depth and in turn
latency) is possible in practice without greatly harming the results.     


==> src/app_softcount.tex <==
\section{Inaccuracies of Soft Counting} \label{app:softcount} 
As outlined in \cref{ssec:eval:warmup}, one reason for an inconsistency between
private and non-private evaluations is the employed soft preliminary counting
heuristic. While this heuristic can cause an inconsistency by inaccurately
predicting the most likely class, it can never lead to an error, \ie an unsound
guarantee.

Recall that the \textsc{Certify} algorithm for randomized smoothing first uses a
heuristic $H$ to guess the top class $k$, which is most likely to be predicted
(see Lines 13\&14 in Algorithm 1). With high probability, \textsc{Certify} will
(i) abstain if the guess was wrong or, (ii) if the guess was correct, abstain or
return the class and a certification radius. In \tool, we use a different
heuristic $H’$, but maintain the same properties: with high probability, if the
result of $H’$ is wrong, the algorithm will abstain and else predict based on
the robustness of the underlying model. Therefore, using $H’$ instead of $H$
does not lead to unsoundness. However, it is possible for $H$ and $H’$ to pick
a different class $k$ for the same input, in which case one heuristic would
predict $k$ while the other would abstain, implying an {inconsistency}. As
we show in \cref{table:results} this is rare in practice.


==> src/building_blocks.tex <==

\section{Our Method} \label{sec:method} 
In this section, we will elaborate the proposed watermarking framework for injecting watermarks into texts written by black-box language models and the corresponding detection process. Table 1 summarizes the notations used in this paper.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.66\linewidth]{CCS2022temp/figures/workflow.pdf}
    \caption{Workflow.}
    \label{fig:workflow}
\end{figure}

\subsection{Framework Overview} %\label{sec:Overview} 
Here, we briefly describe the workflow of our watermarking framework. As shown in Figure \ref{fig:workflow}. Concretely, given a clean enc 

==> src/error.tex <==



\section{Security and Reliability Properties} \label{sec:error}

We now provide a more formal discussion of the properties guaranteed by \tool.
After presenting its security notion (\cref{ssec:error:privacy}), we analyze its
robustness and fairness guarantees (\cref{ssec:error:reliability}).

\subsection{Client Data Privacy} \label{ssec:error:privacy}

As stated in \cref{thm:privacy} below, any passive attacker sitting on the
server or on the network between client and server (see also
\cref{ssec:overview:threat-model}) cannot learn anything about the client data.

\begin{theorem}[Client Data Privacy]\label{thm:privacy}
    A passive polynomial-time attacker with access to all of the server's state
    cannot distinguish two different plaintext inputs $x \neq x'$ of the client.
\end{theorem}

The theorem directly follows from the confidentiality property of
RNS-CKKS~\cite{CheonHKKS18Rns}, assuming hardness of the Ring LWE problem (note
that in \tool, decrypted values are never shared with the server, hence the
attack of \citet{Li2021} does not apply).

\subsection{Robustness and Fairness} \label{ssec:error:reliability}

Recall that in non-private RS (\cref{alg:certify}), a non-abstention result is
robust (\cref{eq:consistency-guarantee}) with probability at least $1-\alpha$,
for some \emph{algorithmic error} probability $\alpha$. In principle, \tool
inherits this guarantee. However, when lifting \cref{alg:certify} to FHE, \tool
introduces an additional \emph{approximation error}, as \textsc{SgnHE} (used
within \textsc{ArgmaxHE}) is only an approximation of \textsc{Sgn} (see
\cref{sec:argmaxhe}).
We analyze this approximation error and bound the total error to
prove \cref{thm:reliability} below.

\begin{theorem}[Reliability] \label{thm:reliability} With high confidence, a
    non-ab\-sten\-tion result returned by \toolR or \toolF satisfies local
    robustness (\cref{eq:consistency-guarantee}) or individual fairness (in the
    form of \cref{eq:robustness2}), respectively, with probability at least
    $1-\xi$, where $\xi$ is computed as described below.
\end{theorem}


Note that \cref{thm:reliability} ignores the additional error introduced by
noise in the RNS-CKKS scheme. However, in line with previous work, \tool
leverages existing error reduction techniques~\cite{BossuatMTH20}  to make these
errors negligible in practice, as we elaborate on in~\cref{ssec:eval:warmup}.
In our evaluation (\cref{sec:eval}), we observe low values of $\xi \leq 0.012$.

In order to prove \cref{thm:reliability}, we next introduce two conditions on
the output logits of the involved neural network. Then, we discuss how we can
upper bound the approximation error probability of \tool by computing the
probability of violating these conditions.

\para{Range and Difference Conditions}
Let $Z_\textit{min}, Z_\textit{max}, D$ be some constants. For all logit vectors
$z \in \mathbb{R}^c$ output by the neural network~$f$ used in \tool, we
introduce the following conditions:
\begin{itemize} 
    \item $\forall i\colon\ z_i \in [Z_\textit{min}, Z_\textit{max}]\ $ (\emph{range
    condition}), and
    \item $\forall i \neq j\colon\ |z_i-z_j| \geq D\ $ (\emph{difference
    condition}).
\end{itemize}

\para{Parameter Selection}
\tool jointly selects \mbox{$(Z_\textit{min}, Z_\textit{max}, D)$}, the
parameters of the \textsc{ArgmaxHE} function \mbox{$(d_{q}^{(1)}$,
$d_{p}^{(1)}$, $d_{q}^{(2)}$, $d_{p}^{(2)})$}, and the precision settings
$(\phi, \psi)$ for each \textsc{SgnHE} invocation such that \emph{zero}
approximation error is introduced if the range and difference conditions hold
(see also~\cref{sec:argmaxhe}). Importantly, choosing $(Z_\textit{min},
Z_\textit{max}, D)$ together with $(\phi, \psi)$ parameters of the first
\textsc{SgnHE} (\cref{lin:argmax:sign-1}) enables us to guarantee that the input
requirement of \textsc{SgnHE} holds, \ie all components of $\mathit{diff}$ are
in $[-1, -\phi] \cup [\phi, 1]$.

While wider $[Z_\textit{min}, Z_\textit{max}]$ and lower $D$ lead to fewer
violations of conditions, this increases the multiplicative depth of the
computation in FHE. In practice, \tool selects a reasonable tradeoff allowing
for both tight error bounds and practical latency. See \appref{app:params} for
full details of the parameter selection procedure.

\para{Bounding the Violation Probability}
To prove \cref{thm:reliability}, it hence suffices to compute an upper bound on
the probability of condition violations. Note that as we empirically observe in
our evaluation~(\cref{sec:eval}), the following derivation is rather loose and
the approximation error gracefully absorbs violations up to some
degree. 

The true range violation probability $\beta_R^\star$ (and analogously $\beta_D
^\star$) can only be computed if the true input distribution is known. However,
as common in machine learning, the true distribution is not known and \tool only
has access to samples from this distribution. To estimate upper bounds $\beta_R$
and $\beta_D$ of $\beta_R^\star$ and $\beta_D^\star$ respectively, \tool relies
on samples from a test set.

First, $\beta_R^\star$ is estimated by $\hat{\beta}_R$, the ratio of examples
$x$ from a test set for which \emph{at least one} of the output logits $z$
violates the range condition. Then, we use the
Clopper-Pearson~\cite{ClopperPearson} confidence interval with p-value $p =
0.05$ to obtain an upper bound $\beta_R$ of $\beta_R^\star$, which holds with
confidence $1 - p$.

We similarly compute an upper bound $\beta_D$ of $\beta_D^\star$: we first
calculate $\hat{\beta}_D$ as the ratio of test set examples for which at least
$\zeta = 1 \%$ of the logits $z$ violate the difference condition, and then
derive $\beta_D$ from $\hat{\beta}_D$ as before, again with confidence $1 - p$.
To ensure soundness when less than a fraction $\zeta$ of the logits~$z$ violate
the condition, we replace $\tau$ with $\tau + \zeta$ in \cref{alg:certify},
following~\cite[Lemma~2]{FischerBV20}.

\begin{proof}[Proof of \cref{thm:reliability}]
Given $\alpha$, $\beta_R$ and $\beta_D$, the total error probability~$\xi$ of
\tool can be computed using the union bound. In particular, with confidence
${1-2p = 0.9}$ (accounting for the two Clopper-Pearson intervals), any
non-abstention value returned by \toolR or \toolF satisfies robustness or
fairness, respectively, except with probability at most ${\xi = \alpha + \beta_R
+ \beta_D}$.
\end{proof}

By using more samples during the estimation of $\beta_R$ and $\beta_D$, we can
decrease $p$ and hence increase the confidence in the theorem.

\para{Unsound Parameters}
In \appref{app:reducing}, we study the effect of selecting unsound parameters
\mbox{$d_{q}^{(1)}$, $d_{p}^{(1)}$, $d_{q}^{(2)}$, $d_{p}^{(2)}$} of
\textsc{ArgmaxHE}. That is, in order to reduce the multiplicative depth of the
FHE computation, we decrease the parameters to purposefully violate the core
\mbox{$(\phi, \psi)$-closeness} property of \textsc{SgnHE} (thus invalidating
\cref{thm:reliability}).

We discover that reducing these parameters below theoretically sound values can
in practice still lead to results consistent with the ones obtained in a
non-private setting, which can be desirable in certain use-cases where formal
guarantees are not essential.


==> src/overview.tex <==
\section{Overview} \label{sec:overview}

We provide a high-level outline of \tool (\cref{ssec:overview:pipeline}),
presenting all algorithmic building blocks needed to enable reliability
guarantees via randomized smoothing. Further, we discuss alternative
instantiations of \tool that enable different properties
(\cref{ssec:overview:guarantees}), its threat model
(\cref{ssec:overview:threat-model}), and why it needs to be deployed on the
server (\cref{ssec:overview:server}).

\subsection{Overview of \tool}
\label{ssec:overview:pipeline}

\tool (\cref{fig:overview}) leverages randomized smoothing to produce ML models
with inference-time reliability guarantees. Key to enabling this in \fhe is to
combine existing techniques for evaluating neural networks in \fhe (marked
``previous work'' in \cref{fig:overview}) with new \fhe counterparts which
handle additional inference-time operations (indicated by (A)--(D) in
\cref{fig:overview}).
In that way, \tool also enables \fhe-execution of any future procedure which
relies on one or more of these fundamental components (as we discuss shortly in
\cref{ssec:overview:guarantees}).

\para{Inference}
The first ingredient is \emph{neural network inference}: Consider a neural
network $f$ classifying an input  $x^{(i)}$ into one of $c$ classes. Concretely,
$f$ outputs a vector of unnormalized scores $z^{(i)}$, called \emph{logits}, and
$f$ is said to classify $x^{(i)}$ to the class with the largest logit.

In the private MLaaS setting, the inputs $x^{(i)}$ are encrypted by the client
using an \fhe scheme (denoted by \lock). Ignoring the addition of noise
(discussed shortly), the inputs are propagated through $f$ utilizing the
homomorphic operations of the \fhe scheme to obtain the logits~$z^{(i)}$. In
\cref{fig:overview}, this is illustrated for $c=3$ where $x^{(1)}$ is classified
to the second class with logit value $z^{(1)}_2 = 2.4$. See
\cref{ssec:background:fhenn} for a more detailed discussion of neural network
inference in \fhe.

\para{Randomized Smoothing}
A core paradigm employed by \tool is \emph{randomized smoothing} (RS, detailed
in \cref{ssec:background:smoothing}). To obtain reliability guarantees, we
\emph{add Gaussian random noise (A)} to many copies of a single input $x^{(1)} =
\dots = x^{(n)}$, and perform neural network inference on these noisy copies to
get a set of logit vectors $z^{(i)}$.

Existing privacy-preserving machine learning systems would typically directly
return the logits~$z^{(i)}$ to the client for decryption
\cite{GiladDLLNW16,BrutzkusGE19,DathathriSCLLMMM19,LouJ21}. However, to apply
RS, \tool includes a \emph{predict step (B)}, which evaluates the \Argmax
function in \fhe. In particular, this step transforms the logit vectors
$z^{(i)}$ of unnormalized scores into \emph{one-hot} vectors $y^{(i)}$ of size
$c$, where a single non-zero entry $y^{(i)}_j$ encodes the index $j$ of the
largest component $z_j^{(i)}$. For example, predicting the second class is
represented by $[0, 1, 0]$. 
  
Next, we \emph{aggregate the predictions (C)} in a statistically sound way
(details given in \cref{sec:smoothing}) to determine the index $k$ of the class
most often predicted by the network, as well as the number of such predictions.

Finally, we perform a homomorphic version of a carefully calibrated
\emph{statistical test (D)}, to obtain $\mathit{ret}$, the ciphertext returned to the client, containing the final prediction with reliability guarantees.


\para{Obtaining Specific Guarantees} Depending on how it is employed, RS is able
to produce different guarantees. In \cref{ssec:smoothing:smoothing}, we discuss
\emph{local robustness} (\toolR), i.e., guaranteeing that minor input
perturbations such as slight changes of lighting conditions for images do not
change the model prediction. Further, in \cref{ssec:smoothing:fairness} we adapt
RS to support inference-time \emph{individual fairness} guarantees (\toolF),
ensuring that similar individuals are treated similarly. 

\subsection{Further Instantiations} \label{ssec:overview:guarantees}

The building blocks (A--D) of RS enabled by \tool are general. Thus, \tool can
also be instantiated in configurations beyond those we consider. In particular,
depending on the number of models used for inference, which subset of
predictions is aggregated, and where noise is added, the output may satisfy
different properties.

Namely, variants of RS have been proposed for various scenarios
\citep{SalmanLRZZBY19, FischerBV20, YangDHSRL20, ChingCAKDG20, FischerBV21,
KumarLF21, BojchevskiKG20, Peychev21}. For example, \citet{Peychev21} combines
RS with generative models to achieve provably fair representation learning, and
\citet{BojchevskiKG20} considers robust reasoning over graphs in the presence of
perturbations on edge weights. To migrate these and similar techniques to \fhe,
the building blocks (A--D) can likely be reused with slight adaptions.

Further, \tool could be instantiated to enhance the privacy properties of
PATE~\cite{PapernotAEGT17}, a state-of-the-art differentially private
learning~\cite{DworkMNS06} framework. In particular, executing PATE in an
FHE-based private setup would preserve the confidentiality of the unlabeled
dataset, making PATE more broadly applicable to scenarios where this data is
private and sensitive. On a technical level, PATE uses an ensemble of models at
the inference step, adding noise~(A) to their aggregated predictions (B--C).
This makes \tool particularly suitable for the task of lifting it to FHE.

Finally, as another example, addition of noise (A) and \Argmax (B) are also
fundamental components of the uncertainty quantification approach proposed by
\citet{Wang19}. 

We leave extending \tool to these settings to future work.


\subsection{Threat Model and Security Notion}\label{ssec:overview:threat-model}

In this work, we consider a combination of two standard threat models: the
two-party semi-honest attacker model from private NN inference (attackers
(i)--(ii) below), and the standard active attacker model from robustness
(attacker (iii) below). In particular, we consider three adversaries: (i) a
semi-honest attacker on the server-side, which tries to learn the plaintext
client input data $x$; (ii)~a semi-honest attacker sitting on the network
between client and server, also trying to learn~$x$; and (iii) an active
adversary on the client-side, which tries to imperceptibly corrupt client's data
$x$. As we will discuss in \cref{ssec:background:robustness}, adversary (iii)
models both naturally occurring measurement errors and deliberate tampering.

The core security notion achieved by \tool is \emph{client data privacy} (see
\cref{thm:privacy} in \cref{ssec:error:privacy}). In particular, we do not aim
to achieve the orthogonal notions of training set privacy or model privacy,
which are concerned with maintaining the privacy of server's data at training
time or maintaining privacy of model data at inference time. Note that attacker
(iii) is irrelevant for ensuring client data privacy. In addition, \tool
satisfies reliability guarantees (see~\cref{thm:reliability} in
\cref{ssec:error:reliability}); only attacker (iii) is relevant for these
properties.

\subsection{Necessity of Computing on the Server}
\label{ssec:overview:server}

\tool executes RS fully on the server. Due to the active client-side adversary
((iii) in \cref{ssec:overview:threat-model}), offloading RS to clients
would make it impossible for the service provider to guarantee reliability, as
such guarantees rely on careful parameter choices and sound execution of the
certification procedure.
For example, in the case of fairness, setting unsuitable parameters of RS on the
client side (maliciously or by accident, both of which are captured by the
active client-side adversary) would allow the clients to use the service to
obtain unfair predictions, nullifying the efforts of the service provider to
prove fairness compliance to external auditors. See
\cref{ssec:error:reliability} for a thorough correctness analysis of guarantees
produced by \tool.

An additional privacy benefit of server-side computation, orthogonal to client
data privacy, is in reducing the threat of \emph{model stealing
attacks}~\cite{TramerZJRR16,ReithST19}, where clients aim to recover the details
of the proprietary model $f$ given the logit vector $z$ of unnormalized scores.
Most prior work on neural network inference in FHE is vulnerable to such attacks
as it returns the encryption of $z$ to the client
\cite{GiladDLLNW16,BrutzkusGE19,DathathriSCLLMMM19,LouJ21}, who then needs to
apply \Argmax on the decrypted vector to obtain the prediction. Merely
approximating the score normalization, \ie executing the softmax function in
FHE~\cite{LeeKLCEDLLYKN21}, was shown to not offer meaningful
protection~\cite{TruongMWP20}. In contrast, applying the approximation of
\Argmax to $z$ in \fhe on the server (as done in \tool) allows the server to
return a one-hot prediction vector to the client. As illustrated by the model
access hierarchy of \citet{JagielskiCBKP20}, this greatly reduces the risk of
model stealing.

Finally, client-side RS would increase the communication cost, as well as the
effort for transitioning existing systems to inference with guarantees or later
modifying the parameters or offered guarantees.

==> src/related_work.tex <==
\section{Related Work} \label{sec:related}

\para{Private Inference via FHE or MPC}
Many recent works consider the problem of neural network inference while
preserving the privacy of client data. To this end, like \tool, many works
instantiate FHE
schemes~\cite{GiladDLLNW16,ChouBLYHF18,BadawiJLMJTNAC21,BrutzkusGE19,LouJ19,LeeKLCEDLLYKN21,LeeLLKKNC21,LouJ21,deepreduce,BouraGGJ20,LuHHMQ20},
while others utilize secure multiparty computation~(MPC) or combine it with
FHE~\cite{PaymanZ17,LiuJLA17,RouhaniRK18,JuvekarVC18,MishraLSZP20,SafeNET,CryptoNAS}.
Both of these research directions are active and growing, with a universally
acknowledged non-comparable set of advantages and drawbacks. As noted in prior
work~\cite{BadawiJLMJTNAC21,BrutzkusGE19,ChouBLYHF18,GiladDLLNW16,deepreduce,LeeLLKKNC21,LeeKLCEDLLYKN21,LouJ19,LouJ21},
MPC-based works have several shortcomings: these approaches typically (i) have
high communication overhead; (ii) require continuous client presence during
inference; (iii) reveal the architecture and model details to the client; (iv)
come with more offline preprocessing (on both client and server); and (v) do not
support large-batch inference. Here, (iii) is often undesirable in a MLaaS
setting. Further, (i), (ii) and (v) are significantly amplified in the setting
of RS, where a large number of inference passes are made for a single client
query.

\para{Reliable Inference} 
A long line of research considers building models with reliability guarantees in
a non-private setting. The two types of guarantees we focus on in \tool are
robustness~\cite{GehrMDCTCV18,GowalDSBQJMK18,WongK18,CohenRK19,FischerBV21}, and
fairness~\cite{DworkHPRZ12,mcnamara2019costs,yeom2020individual,john2020verifying,YurochkinBS20,RuossBFV20}.






\para{Speeding up FHE}
Orthogonal to our work, recent research on optimizing compilers
\cite{BoemerLCW19,DathathriSCLLMMM19,DathathriKSDLM20,ChowdharyDLS21}, GPU
acceleration \cite{DaiS15}, and specialized hardware accelerators for
FHE~\cite{RiaziLPD20,FeldmannSKDDPS22} has demonstrated significant speedups for
FHE. These results suggest that sub-second latencies for \tool are within reach,
which would allow us to investigate more challenging settings in future work.
Specialized hardware will also greatly increase the demand for
privacy-preserving ML solutions, making tools that enable real-world scenarios
in private settings (such as \tool) more valuable.

\para{{Argmax} in FHE} Independent of reliability guarantees for 
ML models, several works discuss lifting \textsc{Argmax} to \fhe.
While \tool targets a non-interactive setting,~\citet{BostPTG15} and
\citet{ChooDDZJPW21} provide interactive protocols for private \textsc{Argmax}.
Works \cite{SebertPZGS21,IliashenkoZ21} discuss the non-interactive evaluation
of \textsc{Argmax} in generally incompatible TFHE~\cite{ChillottiGGI16} and
BGV/BFV~\cite{BrakerskiGV12,FanV12} schemes, thus the proposed constructions
cannot be directly applied to RNS-CKKS. Namely, BGV/BFV operate on integers,
while TFHE operates on bits, has no native support for batched inference, and
offers the concept of ``sign bootstrapping'' leveraged by \citet{SebertPZGS21}
to implement \textsc{Argmax}.
\citet{CheonKKLL19} propose a construction to evaluate \textsc{Argmax} in CKKS,
but this construction is prohibitively expensive~\cite{CheonKK20}. Finally,
\citet{CheonKK20} discuss implementing the \textsc{Max} function via the sign
function approximation, but focus on the simple case of two inputs assumed to be
in $[0,1]$, and thus do not support the significantly more complex general case
of $c>2$ inputs from an unknown domain. In addition, while the FHE engineering
community shows great interest in efficiently evaluating \textsc{Argmax} in
CKKS~\cite{GithubSeal1, GithubSeal2, GithubTenseal1}, no implementation is
publicly available to date.






==> src/smoothing_classification.tex <==
\section{Private Randomized Smoothing}
\label{sec:smoothing} Next, we present how to evaluate RS (see
\cref{ssec:background:smoothing}) in the RNS-CKKS FHE scheme, leveraging
\ArgmaxHE from \cref{sec:argmaxhe}. In particular, we discuss how to
homomorphically execute \cref{alg:certify} and obtain local robustness
guarantees (\toolR, \cref{ssec:smoothing:smoothing}), and how to extend this
approach to guarantee individual fairness (\toolF,
\cref{ssec:smoothing:fairness}).

\subsection{Robustness Guarantees} \label{ssec:smoothing:smoothing}

\toolR instantiates \tool for robustness certification by evaluating
\textsc{Certify} on the server, lifted to \fhe. In the following, we present the
main challenges in achieving this and how \tool overcomes them. First, we
discuss how we implement the \textsc{SampleUnderNoise} subroutine, including the
considerations needed to efficiently execute neural network inference. Then, we
introduce the idea of using \emph{soft preliminary counting} to improve
efficiency, before we describe how to implement the statistical test of
\textsc{Certify}.

\para{Sampling under Noise} The client provides a single encrypted input $x =
[x_0, \ldots, x_d, 0^{M-d}]$ to \toolR. As we require $n$ copies of $x$ in
\cref{lin:certify-noise}, we use a sequence of \texttt{RotR} and $\oplus$
operations to create $n$ duplicated copies $\{x^{(1)}, \ldots, x^{(n)}\}$ of
$x$, packed in $n/B$ ciphertexts as in \cref{eq:xbatch}, where $B = M/(2d)$ is
the batch size. 
Note that all RS parameters, including $n$, are set by the server, \mbox{as noted in \cref{ssec:overview:server}}. 

Next, we independently sample $n$ Gaussian noise vectors
according to \cref{lin:certify-gauss}, and use $\oplus_p$ to homomorphically add
the noise to batched duplicated inputs. We next apply batched neural network
inference, described shortly, to obtain batched logit vectors~$z^{(i)}$, further
reduced to a single ciphertext $\bar{z}$.

\para{Inference} Recall that in the pipeline of \cref{fig:overview}, the inputs
$x^{(i)}$ are encrypted using FHE scheme. To homomorphically evaluate the
neural network $f$ in the inference step (\cref{lin:certify-infer} of
\cref{alg:certify}), we rely on methods from related work discussed in
\cref{ssec:background:fhenn}. Namely, we directly adopt the described approaches
to evaluate $n_\mathit{lin}$ linear and $n_\mathit{act}$ ReLU layers with
multiplicative depth of $\lambda_{\mathit{inf}} = 2 (n_\mathit{lin} +
n_\mathit{act}) - 1$, and heavily utilize SIMD batching, adapting it to our
use-case to reduce the number of expensive FHE operations.

In particular, as commonly $2d \ll M$, we can batch the inputs $x^{(i)}$ in
$M/(2d)$ ciphertexts. Note that this is in contrast to most MLaaS setups, where
inference is typically only performed on a single input at a time and SIMD
batching therefore cannot be effectively utilized~\cite{DathathriSCLLMMM19,
LouJ19}. Next, as inference transforms each $2d$-dimensional input into a
$c$-dimensional logit vector, and commonly $c \ll 2d$, we can further batch the
logit vectors $z^{(i)}$, again using rotations, $\oplus$, and masking of
$\trash$ values using $\otimes_p$ (which adds $\lambda_{\mathit{batching}} = 1$
to the multiplicative depth). This reduces the number of ciphertext inputs to
the costly prediction step (discussed shortly), where it is typically possible
to place all logit vectors into a single ciphertext $\bar{z}$. 


\para{Prediction and Aggregation} For the prediction step
(\cref{lin:certify-argmax-1-hot}), we apply \ArgmaxHE (\cref{sec:argmaxhe}) to
$\bar{z}$ to obtain $\bar{y}$, a ciphertext of batched one-hot prediction
vectors. To aggregate them (\cref{lin:certify-aggregate}), we use a simple
variation of the \emph{RotateAndSum} algorithm~\cite{JuvekarVC18}, which repeatedly
applies rotations and $\oplus$. \textsc{SampleUnderNoise} returns the
ciphertext
\begin{equation*}
    \mathit{counts} = [\mathit{cnt}_1, \ldots, \mathit{cnt}_c, \trash^{M-c}]
\end{equation*}
containing the number of times each class was predicted.


\para{Soft Preliminary Counting}
Determining the most likely class $k$ based on $\mathit{counts}_0$ requires two
invocations of \textsc{ArgmaxHE}
(\cref{lin:certify-argmax-1-hot,lin:certify-argmax2}), significantly increasing
the depth of \textsc{Certify}. 

Recall from \cref{ssec:background:smoothing} that using a heuristic during
preliminary counting does not affect the soundness of RS. Following this, we
introduce the \emph{soft preliminary counting} heuristic. Namely, when computing
$\mathit{counts}_0$, instead of invoking \textsc{ArgmaxHE} to compute one-hot
predictions $y$, we simply rescale $z$ by $1/n$ (by accordingly scaling the
weights of $f$) to obtain a rough approximation of $y$. Consequently, the result
returned in \cref{lin:certify-sample-under-noise-return} holds the average of
all logit vectors.

Avoiding another invocation of \ArgmaxHE greatly reduces the multiplicative
depth of \toolR, which would otherwise be prohibitive. At the same time, soft
counting does not affect the soundness of the guarantees, and as we demonstrate
in \cref{sec:eval}, it rarely impacts the decisions of \textsc{Certify}. See
\appref{app:softcount} for further discussion.



\para{Statistical Testing}
We next describe how to evaluate the statistical test in
\crefrange{lin:certify-binp}{lin:certify-return-abstain}, which provides a robustness guarantee.

Let $p_k$ denote the probability that the smoothed model~$G$
(\cref{eq:smoothed}) predicts $k$ as computed in \cref{lin:certify-argmax2}. The
one-sided binomial test attempts to prove that $p_k > \tau$ with error
probability at most $\alpha$. To this end, it computes the $p$-value \mbox{$pv =
1 - \textsc{BinCDF}(\mathit{counts}[k]-1; n, \tau)$}, the probability of
predicting the class $k$ at least $\mathit{counts}[k]$ out of $n$ times under
the worst case $p_k=\tau$ of the null hypothesis $p_k \leq \tau$, where
$\textsc{BinCDF}$ denotes the binomial CDF. 

Computing $\textsc{BinCDF}$ on $\mathit{counts}[k]$ involves approximating the
incomplete beta function, which is not easily reducible to FHE primitives. To
overcome this, we rephrase the test using the following observation: For fixed
$n$ and $\tau$, the \mbox{p-value} $pv$ is strictly decreasing \wrt
$\mathit{counts}[k]$. Thus, we employ binary search to find $\mathit{target}$,
the smallest value of $\mathit{counts}[k]$ for which $pv \leq \alpha$, \ie the
test passes. We visualize this in \cref{fig:bintest}, where $k = 3$, and
$\mathit{target} = 6$.

\begin{figure}
    \centering
    \includegraphics[width=0.65\linewidth]{figures/bintest.pdf}
    \caption{The statistical test of \tool, illustrated on an example.} 
    \label{fig:bintest}
\end{figure}

Let $k_\mathit{1hot}$ denote the one-hot vector encoding the predicted class,
obtained by multiplying the result of \textsc{ArgmaxHE} in
\cref{lin:certify-argmax2} with $[1^c, 0^{M-c}]$ using $\otimes_p$, such that
the non-zero slot is at index $k$. The server returns a ciphertext
$\mathit{ret}$ to the client, computed as follows:
\begin{equation} \label{eq:ret}
    \mathit{ret} \leftarrow k_{\mathit{1hot}} \otimes (\mathit{counts} \ominus_p \mathit{shift}),
\end{equation}
where \mbox{$\mathit{shift} = [(\mathit{target}-1)^c, 0^{M-c}]$} is the
plaintext with $\mathit{target}-1$ in first $c$ slots, and $0$ in rest. Note
that the use of $\otimes_p$ to obtain $k_{1hot}$ and the use of $\otimes$ in
\cref{eq:ret} add $\lambda_{ret} = 2$ to multiplicative depth. We illustrate the
computation of $\mathit{ret}$ in \cref{fig:bintest}, where $M = 4$ and $c = 3$. 

\para{Interpreting the Result} The client decrypts and decodes $\mathit{ret}$
using the secret key, rounds all its entries to the closest integer value, and
finds $Z$, the unique non-zero value in first $c$ slots of~$\mathit{ret}$. If
such a $Z$ does not exist (\ie $\mathit{counts}[k] = target-1$), we define $Z =
0$. In \cref{fig:bintest} it is $Z=4$ at slot $k=3$.
There are two possible outcomes.


\begin{itemize}
    \item \emph{Abstention}: If $Z\leq 0$, the prediction is to be discarded, as
    robustness cannot be guaranteed.
    \item \emph{Guarantee}: If $Z>0$, the model predicts $k$ and is guaranteed
    to be robust in the $\ell_2$ ball of radius $R$ around the input $x$
    (\cref{eq:consistency-guarantee}) with probability at least $1-\xi$
    (discussed below), where $R$ and $\xi$ can be communicated to the client
    unencrypted.
\end{itemize}
Note that if necessary, the server can avoid revealing the predicted class in
the \emph{abstention} case, and the value of $Z$, by appropriately rescaling $Z$
within $\mathit{ret}$ and applying another \textsc{SgnHE}, such that
$\mathit{ret}$ is one-hot if the outcome is guaranteed to be robust, and the
all-zero vector otherwise. In our implementation, we omit this step to avoid
increasing the multiplicative depth.

The non-homomorphic version of RS (\cref{alg:certify}) ensures robustness with
probability at least $1-\alpha$ if it does not return ``abstain''. As the
homomorphic version in \toolR includes various approximations, it introduces an
additional approximation error, resulting in a total error probability bound
$\xi$ (discussed in~\cref{sec:error}).

\para{Multiplicative Depth} Summing up previously derived depths of inference,
batching, \textsc{ArgmaxHE}, and the calculations in \cref{eq:ret}, we obtain
the total multiplicative depth of \toolR: 
\begin{align*}
    \lambda &= \lambda_{\mathit{inf}} + \lambda_{\mathit{batching}} + \lambda_{\mathit{argmax}} + \lambda_{\mathit{ret}} \\ 
    &= 2(n_\mathit{lin} + n_\mathit{act}) + 4(d_q^{(1)}+d_p^{(1)} + d_q^{(2)}+d_p^{(2)}) + 3.
\end{align*}
An extensive experimental evaluation given in \cref{ssec:eval:smoothing}
demonstrates that this leads to practical latency.





==> src/smoothing_fairness.tex <==
\subsection{Individual Fairness Guarantees}
\label{ssec:smoothing:fairness}
Next, we present how \toolF instantiates \tool for individual fairness
guarantees by applying a generalization of RS.

\para{Metric Fairness as Robustness}
Inspired by \citet{YurochkinBS20,MukherjeeYBS20} and \citet{RuossBFV20}, we
transform the definition of metric fairness (\cref{eq:metric_fairness}) into a
variant of local robustness (\cref{eq:consistency-guarantee}), allowing us to
utilize RS to obtain guarantees. Similar to \cite{YurochkinBS20,MukherjeeYBS20},
we consider input space metrics of the form
\begin{equation*} 
  d_{x}(x_{1}, x_{2}) := \left(x_{1} - x_{2} \right)^{\top} \Theta \left(x_{1} - x_{2}\right),
\end{equation*}
where $\Theta$ is a symmetric positive definite matrix. We focus on classifiers,
thus we have $\mathcal{Y} = [c]$ in \cref{eq:metric_fairness}, and $d_{y}(y_{1}, y_{2})
:= \indicator{y_{1} \neq y_{2}}$, \ie $d_{y}(y_{1}, y_{2}) = 1$ if $y_{1} \neq
y_{2}$, and $0$ otherwise.

For fixed $x$, to show that $F$ is individually fair, we need to show:
\begin{equation}
  \label{eq:lipp_fair_simple}
  \forall x' \in \mathcal{X}\colon \quad \indicator{F(x) \neq F(x')} \leq L \left(x - x'\right)^{\top} \Theta \left(x - x'\right).
\end{equation}
We let $\|x\|_{\Theta} := \sqrt{x^{\top} \Theta x}$ denote the Mahalanobis norm and
rewrite \cref{eq:lipp_fair_simple} as
\begin{align}
  & \forall x' \in \mathcal{X}\colon \quad F(x) \neq F(x') \implies \|x-x'\|_{\Theta}^{2} \geq 1/L \nonumber \\
  \iff & \forall x' \in \mathcal{X}\colon \quad \|x-x'\|_{\Theta}^{2} < 1/L \implies F(x) = F(x') \nonumber \\
  \iff &\forall \delta \; \text{with} \; \|\delta\|_{\Theta} < \sqrt{1/L}\colon \quad F(x) = F(x + \delta),
  \label{eq:robustness2}
\end{align}
which represents a local robustness constraint (\cref{eq:consistency-guarantee})
with radius $R=\sqrt{1/L}$, and the $\ell_2$ norm generalized to the
$\|\cdot\|_{S}$ norm.

In other words, by achieving Mahalanobis norm robustness, we can achieve
equivalent individual fairness guarantees.

\para{Similarity Constraint} To set $\Theta$ and $L$, we choose the
\emph{similarity constraint} $\theta \in \mathbb{R}^d$, encoding the
problem-specific understanding of similarity. Concretely, $\theta_i$ is chosen
to quantify the minimum difference in attribute $i$ (\eg client age in our
example of fair loan eligibility prediction from \cref{sec:motivation}) for
which two individuals are considered dissimilar, assuming all other attributes
are fixed.

The similarity constraint should be set by a data regulator \cite{DworkHPRZ12,
McNamaraOW17}. In our analysis, following prior work on fairness certification
\cite{RuossBFV20,john2020verifying}, we consider the problem of choosing the
similarity constraint orthogonal to this investigation and assume it to be
given.

Given $\theta$, we set $\Theta = diag(1/\theta^2)$, where squaring is applied
componentwise, and $L=1$, which implies $R = \sqrt{1/L}=1$. Intuitively, for two
individuals differing only in attribute $i$ by $\delta < s_i$, we will have
$\|\delta\|_{\Theta} < 1 = R$, \ie to ensure fairness, the prediction of the
model $F$ should be the same for these individuals, as per
\cref{eq:lipp_fair_simple}.

\para{Mahalanobis Randomized Smoothing}
To produce individual fairness guarantees via Mahalanobis norm robustness,
\toolF leverages a generalization of RS from \citet[Theorem A.1]{FischerBV20}.
In particular, the noise added before the inference step is sampled from
$\mathcal{N}(0, \Sigma)$ instead of $\mathcal{N}(0, \sigma^2 I_d)$, where
$\Sigma$ is a covariance matrix. If the algorithm does not return the
``abstain'' decision, the returned class $k$ satisfies the following robustness
guarantee:
\[
  \forall \delta \text{ with } \|\delta\|_{\Sigma^{-1}} < R: \quad G(x + \delta) = k,
\]
where $G$ denotes the smoothed classifier to be used instead of $F$ (see
\cref{ssec:background:smoothing}), and $R= \Phi^{-1}(\tau)$, for $\tau$ and
$\Sigma$ being parameters of RS.
 
Given $\Theta$ and $L$, instantiating this with $\Sigma = \Theta^{-1}$ and $\tau
= \Phi(\sqrt{1/L})$ implies $R=\sqrt{1/L}$ and recovers \cref{eq:robustness2},
directly leading to individual fairness guarantees with respect to our
similarity constraint. 

Therefore, by changing the distribution of the noise applied to the inputs in
\toolR as part of RS, we obtain \toolF. An experimental evaluation of \toolR and
\toolF is given in \cref{sec:eval}.



==> tables/app_reducing.tex <==
\begin{table}[t]\centering

    \caption{MockSEAL evaluation of private inference with robustness guarantees
    on the MNIST dataset with less polynomial evaluations within the
    \textsc{SgnHE} approximation. We show consistency with the non-private
    evaluation (in \%) at count and result level.} 
    \label{table:reducing}
    
    \newcommand{\twocol}[1]{\multicolumn{2}{c}{#1}}
    \newcommand{\fivecol}[1]{\multicolumn{5}{c}{#1}}
    \renewcommand{\arraystretch}{1.2}
   
  
    \begin{tabular}{@{}ccccrr@{}} \toprule
    $d_q^{(1)}$ & $d_p^{(1)}$ & $d_q^{(2)}$ & $d_p^{(2)}$ & CountsOK & ResultOK  \\ \cmidrule{1-6}
    6 & 1 & 2 & 2 & 100.00 & 100.00 \\
    \midrule 
    6 & 1 & 2 & 1 & 100.00 & 99.99 \\
    6 & 1 & 2 & 0 & 0.00 & 0.00 \\
    6 & 1 & 1 & 2 & 5.97 & 1.89 \\
    6 & 1 & 0 & 2 & 0.00 & 0.00 \\
    6 & 0 & 2 & 2 & 0.00 & 13.92 \\
    5 & 1 & 2 & 2 & 99.93 & 99.99 \\
    5 & 1 & 2 & 1 & 99.88 & 99.98 \\
    4 & 1 & 2 & 2 & 99.20 & 99.97 \\
    4 & 1 & 2 & 1 & 98.66 & 99.92 \\
    3 & 1 & 2 & 2 & 89.63 & 99.77 \\
    3 & 1 & 2 & 1 & 87.49 & 99.52 \\
    2 & 1 & 2 & 2 & 60.93 & 97.15 \\
    2 & 1 & 2 & 1 & 58.69 & 96.02 \\
    1 & 1 & 2 & 2 & 3.00 & 25.48 \\
    1 & 1 & 2 & 1 & 2.53 & 24.85 \\
    \bottomrule  
    \end{tabular}
\end{table}
  

==> tables/latency.tex <==
\begin{table*}[t]\centering

  \caption{The evaluation of performance. Each row represents a parameter
  variation of the baseline experimental setting (MNIST model). For each of the
  main components of \toolR, we report the mean latency of 10 runs, as well as
  the relative cost in isolation (see \cref{ssec:eval:latency}).}
  \label{table:latency}
  
  \newcommand{\twocol}[1]{\multicolumn{2}{c}{#1}}
  \renewcommand{\arraystretch}{1.2}


  \resizebox{0.65 \linewidth}{!}{
  \begin{tabular}{@{}rrrrrrr@{}} \toprule

  & (i)~Duplication & (ii)~Inference & \multirow{2}{*}{(iii)~\textsc{ArgmaxHE}}
  & (iv)~Aggregation && \multirow{2}{*}{Total} \\ 
  
  & + Noise & + Reduction &  & + BinTest &&  \\ \midrule

  Baseline & 37s (1.0) & 662s (191.0) & 157s (\phantom{0}84.5) & <1s (1.4) && 856s (277.9) \\ \midrule
  $1/2$ Data Size & 41s (1.0) & 608s (\phantom{0}98.6) & 157s (\phantom{0}72.8) & <1s (1.2) && 806s (173.6) \\
  $2 \times$ Data Size & 33s (1.0) & 740s (408.7) & 156s (100.2) & <1s (1.6) && 929s (890.1) \\
  $-1$ Layers & 31s (1.0) & 233s (\phantom{0}62.0) & 159s (\phantom{0}84.5) & <1s (1.4) && 424s (148.9) \\
  $+1$ Layers & 43s (1.0) & 1734s (466.5) & 158s (\phantom{0}84.5) & <1s (1.4) && 1935s (553.4) \\
  $1/2$ Width & 37s (1.0) & 431s (119.6) & 159s (\phantom{0}84.5) & <1s (1.4) && 628s (206.5) \\
  $2 \times$ Width & 37s (1.0) & 1177s (337.5) & 158s (\phantom{0}84.5) & <1s (1.4) && 1371s (424.4) \\

  \bottomrule 
  \end{tabular}}

\end{table*} 


==> tables/nets.tex <==
\begin{table}[t]\centering

    \caption{Overview of the models used in consistency experiments.}
    \label{table:nets}
    
    \newcommand{\twocol}[1]{\multicolumn{2}{c}{#1}}
    \renewcommand{\arraystretch}{1.2}
  
  
    \resizebox{\columnwidth}{!} {
    \begin{tabular}{@{}rrrrrrrr@{}} \toprule
    & Acc ($\%$) & $R$ & Cert ($\%$)&  $Z_\textit{min}$ & $Z_\textit{max}$ & D &$\xi$\\ \midrule
    MNIST  & 96.8 & 0.34 & 86.1 & -80 & 60 & 0.0056& 0.0028 \\
    CIFAR   & 52.7 & 0.17 & 47.7& -10 & 45 & 0.0022 & 0.0120  \\
    Adult  & 81.6 & n/a & 95.7& -180 & 180 & 0.0072 & 0.0014 \\
    \midrule 
    MNIST{$_{\sigma=0.75}$}   & 95.5  & 0.34 & 78.8& -40 & 50 & 0.0036 & 0.0016\\
    MNIST{$_{\sigma=1.0}$}   & 94.3 & 0.34 & 68.1& -30 & 45 & 0.0030& 0.0016   \\
    MNIST{$_{\sigma=1.5}$}   & 91.3 & 0.34 & 44.0& -25 & 30 & 0.0022 & 0.0018\\
    MNIST{$_{\eta=2.0}$}  & 93.25 & 0.5 & 62.1 & -35 & 50 & 0.0034& 0.0032  \\
    \bottomrule %
    \end{tabular}}
  \end{table} 
  

==> tables/results.tex <==
\begin{table*}[t]\centering

    \caption{Evaluation of private inference with guarantees with \tool on
    models from \cref{table:nets}. We show the validity of results obtained in
    FHE, and the consistency (in \%) with the non-private evaluation at
    prediction, count, and result level (see \cref{ssec:eval:smoothing}).
    Further, we show the fraction of (harmful; H) range violations (RV) and
    difference violations (DV). P- denotes the violations during the process of
    preliminary counting.}
    \label{table:results}
    
    \newcommand{\twocol}[1]{\multicolumn{2}{c}{#1}}
    \renewcommand{\arraystretch}{1.2}
  
  
    \resizebox{0.77\linewidth}{!} {
    \begin{tabular}{@{}rrrrrrrrr@{}} \toprule
    Model & Valid1Hot & PredOK & CountsOK & ResultOK & RV (H) & DV (H) & P-RV (H) & P-DV (H) \\ \midrule
    MNIST--MockSEAL & 100.00& 99.52 & 100.00 & 100.00 & 0.00 (0.00) & 92.08 (5.05) & 0.00 (0.00) & 2.23 (0.02) \\ 
    MNIST--SEAL & 100.00 & 100.00 & 100.00 & 100.00 & 0.00 (0.00) & 97.06 (7.84) & 0.00 (0.00) & 5.88 (0.00) \\
    CIFAR--MockSEAL& 99.99 & 94.71 & 99.97 & 99.98 & 0.22 (0.00) & 77.49 (11.68) & 0.05 (0.00) & 2.75 (0.22) \\
    CIFAR--SEAL& 100.00& 97.00 & 100.00& 100.00& 0.00 (0.00) & 82.00 (11.00) & 0.00 (0.00) & 3.00 (0.00) \\
    Adult--MockSEAL & 99.98 & 99.89 & 98.42 & 99.97 & 0.00 (0.00) & 29.41 (29.41) & 0.00 (0.00) & 0.12 (0.12) \\
    Adult--SEAL & 100.00 & 100.00 & 95.00 & 100.00 & 0.00 (0.00) & 58.00 (58.00) & 0.00 (0.00) & 0.00 (0.00) \\
    \midrule 
    MNIST{$_{\sigma=0.75}$}--MockSEAL & 100.00& 98.82 & 99.96 & 100.00& 0.00 (0.00) & 89.32 (6.57) & 0.00 (0.00) & 2.09 (0.00) \\
    MNIST{$_{\sigma=1.0}$}--MockSEAL & 100.00& 97.93 & 99.98 & 100.00& 0.00 (0.00) & 91.58 (9.28) & 0.00 (0.00) & 2.53 (0.08) \\
    MNIST{$_{\sigma=1.5}$}--MockSEAL & 99.99 & 95.42 & 99.96 & 99.99 & 0.00 (0.00) & 94.35 (12.88) & 0.00 (0.00) & 3.09 (0.07) \\
    MNIST{$_{\eta=2.0}$}--MockSEAL  & 99.99 & 97.35 & 99.98 & 99.99 & 0.00 (0.00) & 96.4 (13.56) & 0.00 (0.00) & 3.49 (0.03) \\
    \bottomrule 
    \end{tabular}}
  \end{table*} 
  
